A Long Short-Term Memory for AI Applications in Spike-based Neuromorphic Hardware

Spike-based neuromorphic hardware holds the promise to provide more energy efficient implementations of Deep Neural Networks (DNNs) than standard hardware such as GPUs. But this requires to understand how DNNs can be emulated in an event-based sparse firing regime, since otherwise the energy-advantage gets lost. In particular, DNNs that solve sequence processing tasks typically employ Long Short-Term Memory (LSTM) units that are hard to emulate with few spikes. We show that a facet of many biological neurons, slow after-hyperpolarizing (AHP) currents after each spike, provides an efficient solution. AHP-currents can easily be implemented in neuromorphic hardware that supports multi-compartment neuron models, such as Intel's Loihi chip. Filter approximation theory explains why AHP-neurons can emulate the function of LSTM units. This yields a highly energy-efficient approach to time series classification. Furthermore it provides the basis for implementing with very sparse firing an important class of large DNNs that extract relations between words and sentences in a text in order to answer questions about the text.

==> tab/bench_table.tex <==
%!TEX root = ../main.tex
% Edited table in following site https://www.latex-tables.com/
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}
\centering
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\label{tab:sMNIST-power-results}
\arrayrulecolor{black}
\begin{tabular}{c|c|c|c|c|c}
\textbf{}                                                                                   & \textbf{\# sentences}                                     & \textbf{batch size}   & \textbf{Latency ratio}  & \textbf{Energy ratio}  & \textbf{EDP ratio}    \\
\textbf{Hardware}                                                                           & \textbf{\# cores}                                         & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}  & \multicolumn{1}{l}{}  \\ 
\hline
Loihi                                                                                       & \begin{tabular}[c]{@{}c@{}}20\\ 2320 cores \end{tabular}  & 1                     & 1.00x                   & 1.00x                  & \textbf{1.00x}        \\ 
\arrayrulecolor[rgb]{0.714,0.714,0.714}\hline
\rowcolor[rgb]{0.8,0.8,0.8} {\cellcolor[rgb]{0.8,0.8,0.8}}                                  & {\cellcolor[rgb]{0.8,0.8,0.8}}                            & 1                     & 0.38x                   & 4.36x                  & \textbf{1.67x}        \\
\rowcolor[rgb]{0.8,0.8,0.8} \multirow{-2}{*}{{\cellcolor[rgb]{0.8,0.8,0.8}}Nvidia RTX 2070} & \multirow{-2}{*}{{\cellcolor[rgb]{0.8,0.8,0.8}}20}        & 100                   & 1.26x                   & 0.42x                  & 0.53x                 \\ 
\arrayrulecolor{black}\midrule
Loihi                                                                                       & \begin{tabular}[c]{@{}c@{}}16*\\ 1552 cores \end{tabular} & 1                     & 1.00x                   & 1.00x                  & \textbf{1.00x}        \\ 
\arrayrulecolor[rgb]{0.714,0.714,0.714}\hline
\rowcolor[rgb]{0.8,0.8,0.8} {\cellcolor[rgb]{0.8,0.8,0.8}}                                  & {\cellcolor[rgb]{0.8,0.8,0.8}}                            & 1                     & 0.33x                   & 5.32x                  & \textbf{1.73x}        \\
\rowcolor[rgb]{0.8,0.8,0.8} \multirow{-2}{*}{{\cellcolor[rgb]{0.8,0.8,0.8}}Nvidia RTX 2070} & \multirow{-2}{*}{{\cellcolor[rgb]{0.8,0.8,0.8}}16}        & 100                   & 0.68x                   & 0.31x                  & 0.21x                 \\ 
\arrayrulecolor{black}\midrule
Loihi                                                                                       & \begin{tabular}[c]{@{}c@{}}10\\ 700 cores \end{tabular}   & 1                     & 1.00x                   & 1.00x                  & \textbf{1.00x}        \\ 
\arrayrulecolor[rgb]{0.714,0.714,0.714}\hline
\rowcolor[rgb]{0.8,0.8,0.8} {\cellcolor[rgb]{0.8,0.8,0.8}}                                  & {\cellcolor[rgb]{0.8,0.8,0.8}}                            & 1                     & 0.44x                   & 7.78x                  & \textbf{3.41x}        \\
\rowcolor[rgb]{0.8,0.8,0.8} \multirow{-2}{*}{{\cellcolor[rgb]{0.8,0.8,0.8}}Nvidia RTX 2070} & \multirow{-2}{*}{{\cellcolor[rgb]{0.8,0.8,0.8}}10}        & 100                   & 0.76x                   & 0.35x                  & 0.27x                 \\ 
\arrayrulecolor{black}\midrule
Loihi                                                                                       & \begin{tabular}[c]{@{}c@{}}6\\ 332 cores \end{tabular}    & 1                     & 1.00x                   & 1.00x                  & \textbf{1.00x}        \\ 
\arrayrulecolor[rgb]{0.714,0.714,0.714}\hline
\rowcolor[rgb]{0.8,0.8,0.8} {\cellcolor[rgb]{0.8,0.8,0.8}}                                  & {\cellcolor[rgb]{0.8,0.8,0.8}}                            & 1                     & 0.56x                   & 11.92x                 & \textbf{6.73x}        \\
\rowcolor[rgb]{0.8,0.8,0.8} \multirow{-2}{*}{{\cellcolor[rgb]{0.8,0.8,0.8}}Nvidia RTX 2070} & \multirow{-2}{*}{{\cellcolor[rgb]{0.8,0.8,0.8}}6}         & 100                   & 0.95x                   & 0.44x                  & 0.42x                 \\ 
\arrayrulecolor{black}\midrule
Loihi                                                                                       & \begin{tabular}[c]{@{}c@{}}2\\ 124 cores \end{tabular}    & 1                     & 1.00x                   & 1.00x                  & \textbf{1.00x}        \\ 
\arrayrulecolor[rgb]{0.502,0.502,0.502}\hline
\rowcolor[rgb]{0.8,0.8,0.8} {\cellcolor[rgb]{0.8,0.8,0.8}}                                  & {\cellcolor[rgb]{0.8,0.8,0.8}}                            & 1                     & 0.73x                   & 16.49x                 & \textbf{12.10x}       \\
\rowcolor[rgb]{0.8,0.8,0.8} \multirow{-2}{*}{{\cellcolor[rgb]{0.8,0.8,0.8}}Nvidia RTX 2070} & \multirow{-2}{*}{{\cellcolor[rgb]{0.8,0.8,0.8}}2}         & 100                   & 1.06x                   & 0.50x                  & 0.53x                
\end{tabular}
\arrayrulecolor{black}
\caption{Benchmarking comparison and scaling analysis of the spiking relational network on Loihi against the corresponding ANN on GPU\protect\footnotemark. The data set was grouped by number sentences per sample which in turn determines the number of AHP-SNNs and therefore cores per sample. All measurements were done using 250 input samples *except for network size 16 were only 100 samples were used, as there are not enough test samples containing 16 sentences. The energy per inference was calculated using total power values.}
\end{table}

\footnotetext{Loihi: Nahuku board (ncl-ghrd-01), CPU: Intel Core i9-7920X, RAM: 128GB, OS: Ubuntu 16.04.6 LTS, NxSDK: 0.95\\
Nvidia RTX 2070: Nvidia RTX 2070 Super, GPU-RAM: 8GB, CPU: Intel Core i7-9700K, RAM: 32GB, OS: Ubuntu 16.04.6 LTS, Python 3.6.5, TensorFlow-GPU: 1.14.0, CUDA: 10.0.\\
Intel Core i5-7440HQ: RAM: 16GB, OS: Windows 10 (build18362), Python 3.6.7, TensorFlow: 1.14.1\\
Performance results are based on testing as of \today{} and may not reflect all publicly available security updates. Results may vary.}

==> tab/sMNIST_hyperparameters.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{@{}lll@{}}
\toprule
                       & original LSNN & AHP-SNN on Loihi     \\ \midrule
$\beta$   & 1.8           & 1390000        \\
baseline threshold $b^0$        & 0.01          & 8128           \\
refractory steps       & 5 ms          & 1              \\
number of delays       & 10            & 1              \\
$\tau_m$ & 20 ms         & 20 time steps  \\
$\tau_a$ & 700 ms        & 700 time steps \\
scaling constant $\zeta$       & -             & 620            \\ \bottomrule
\end{tabular}
\caption{Hyper-parameters of the original LSNN model and the corresponding hyper-parameters of the AHP-SNN on Loihi.}
\label{tab:sMNIST-hyperparameters}
\end{center}
\end{table}
